Free Proxies Unmasked: A Vulnerability and Longitudinal Analysis of Free Proxy Services

Free-proxies have been widespread since the early days of the Web, helping users bypass geo-blocked content and conceal their IP addresses. Various proxy providers promise faster Internet or increased privacy while advertising their lists comprised of hundreds of readily available free proxies. However, while paid proxy services advertise the support of encrypted connections and high stability, free proxies often lack such guarantees, making them prone to malicious activities such as eavesdropping or modifying content. Furthermore, there is a market that encourages exploiting devices to install proxies. In this paper, we present a 30-month longitudinal study analyzing the stability, security, and potential manipulation of free web proxies that we collected from 11 providers. Our collection resulted in over 640,600 proxies, that we cumulatively tested daily. We find that only 34.5% of proxies were active at least once during our tests, showcasing the general instability of free proxies. Geographically, a majority of proxies originate from the US and China. Leveraging the Shodan search engine, we identified 4,452 distinct vulnerabilities on the proxies' IP addresses, including 1,755 vulnerabilities that allow unauthorized remote code execution and 2,036 that enable privilege escalation on the host device. Through the software analysis on the proxies' IP addresses, we find that 42,206 of them appear to run on MikroTik routers. Worryingly, we also discovered 16,923 proxies that manipulate content, indicating potential malicious intent by proxy owners. Ultimately, our research reveals that the use of free web proxies poses significant risks to users' privacy and security. The instability, vulnerabilities, and potential for malicious actions uncovered in our analysis lead us to strongly caution users against relying on free proxies.

==> sections/3_related_works.tex <==
\section{Related work}

The recent years saw a rise in the number of papers focusing on the free proxy ecosystem.  Tsirantonakis~\etal{}~\cite{tsirantonakis2018large} were the first to perform a large-scale analysis of open proxies. Through the probing of over 65,000 proxies over a two months period, they find that over 38\% of working proxies perform some kind of content modification. However, they stress that only a small subset of these proxies do in fact alter the expected content in a malicious way. 

Mani~\etal{}~\cite{mani2018extensive} follow the same methodology in their proxy analysis and provide insights obtained through a 50-day study of over 107,000 open proxies. They found that even though the open proxies may be geographically diverse, only a few countries account for the majority of working proxies. Another key finding in their study shows that content-manipulating proxies rarely induce harmful impacts, however, when it is a proxy's motive, it can go as far as introducing cryptocurrency mining scripts and forcing trojans executables to the users. Finally, Mani~\etal{} enriches their study by analyzing content manipulation over a Tor network.

ProxyTorrent~\cite{perino2018proxytorrent} builds on the previous works and extends the study to over 180,000 free proxies over 10 months while providing a more precise analysis of the ecosystem by considering TLS certificate manipulation and emphasizing proxy performance. ProxyTorrent also provided a web extension through which users could select a secure free proxy suiting their needs. The extension allowed the study to look over the free proxy ecosystem through a unique point of view and better characterize the extent of selective data manipulation from the free proxies.

Finally, Choi~\etal{}~\cite{choi2020understanding} performed the largest open proxies analysis to date, collecting over 7,000,000 proxies, of which over 1,000,000 are open proxies. While the main purpose of their study is to compare open proxies to residential proxies, they provide a precise overview of the reliability of open proxies on the Internet.


